A 5G-Edge Architecture for Computational Offloading of Computer Vision Applications

Processing computer vision applications (CVA) on mobile devices is challenging due to limited battery life and computing power. While cloud-based remote processing of CVA offers abundant computational resources, it introduces latency issues that can hinder real-time applications. To overcome this problem, computational offloading to edge servers has been adopted by industry and academic research. Furthermore, 5G access can also benefit CVA with lower latency and higher bandwidth than previous cellular generations. As the number of Mobile Operators and Internet Service providers relying on 5G access is growing, it is of paramount importance to elaborate a solution for supporting real time applications with the assistance of the edge computing. Besides that, open-source based platforms for Multi-access Edge Computing (MEC) and 5G core can be deployed to rapid prototyping and testing applications. This paper aims at providing an end-to-end solution of open-source MEC and 5G Core platforms along with a commercial 5G Radio. We first conceived a 5G-edge computing environment to assist near to user processing of computer vision applications. Then a sentiment analysis application is developed and integrated to the proposed 5G-Edge architecture. Finally, we conducted a performance evaluation of the proposed solution and compare it against a remote cloud-based approach in order to highlight the benefits of our proposal. The proposed architecture achieved a 260\% throughput performance increase and reduced response time by 71.3\% compared to the remote-cloud-based offloading.

==> Textos/trabalhosRelacionados.tex <==
\section{Related Work}
\label{sec:relWork}

This session presents the state of the art in terms of using MEC platforms for critical deployments that require real-time processing, and also highlights the importance of using remote processing instead of local processing. 

% The Table \ref{tab:rel_work} summarizes the related work, highlighting the layer at which the data is actually processed, the application used, the evaluation environment, and the study's objective.

% \begin{table*}
%   \caption{Related Work Summary}
%   \label{tab:rel_work}
%   \begin{tabular}{cccccl}
%     \toprule
%     Paper & Processing Layer & Application Type & Environment & Objective\\
%     \midrule
%     %\cite{Demo} & MEC & Computer Vision & 5G Testbed & Remote processing to Vehicle-to-everything (V2X) scenarios  \\
%     \cite{UAV} & MEC/Local & Computer Vision & 4G Testbed & Performance and energy efficiency analysis on UAVs offloading\\
%     \cite{mar_edge} &  Local/Cloud/Edge & Augmented Reality & Simulation & Performance and energy efficiency analysis on AR apps offloading\\
    

%     This Paper & MEC/Cloud & Computer Visions & 5G Testbed & Remote processing of computer vision algorithms with MEC and 5G\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% O trabalho apresentado por \cite{Demo} demonstra um protótipo de detecção de objetos em Veículo Cooperativo para Tudo (CV2X) utilizando dados de vídeo. A demonstração utiliza o núcleo 5G (5GC) da Capgemini acoplado a um servidor de borda para alcançar comunicação de baixa latência. O sistema emprega o algoritmo de detecção de objetos YOLO em servidores de borda para processar vídeos capturados por veículos em um ambiente 5G com mobilidade de borda. A plataforma proprietária utilizada na demonstração, apesar de apresentar benefícios, falha em realizar uma avaliação de desempenho quantitativa e não fornece uma análise comparativa com outras abordagens, inclusive com a computação em nuvem.
%The work presented by \cite{Demo} demonstrates a prototype for object detection in Cooperative Vehicle-to-Everything (CV2X) using video data. The demonstration utilizes Capgemini's 5G Core (5GC) coupled with an edge server to achieve low-latency communication. The system employs the YOLO object detection algorithm on edge servers to process videos captured by vehicles in a 5G environment. While the proprietary platform used in the demonstration offers advantages, it fails to conduct a quantitative performance evaluation and lacks a comparative analysis with alternative approaches, including cloud computing.

%A proposta apresentada por \cite{UAV} explora o potencial de Veículos Aéreos Não Tripulados (UAVs) equipados com dispositivos IoT para vigilância por reconhecimento facial em grandes altitudes. O estudo demonstra a viabilidade de offloading de tarefas de processamento de dados de vídeo para servidores mobile edge computing (MEC), reduzindo o consumo de energia e o tempo de processamento a bordo dos UAVs. O trabalho apresenta um protótipo para reconhecimento facial utilizando o algoritmo Local Binary Pattern Histogram (LBPH) do OpenCV em um ambiente de teste. Os resultados demonstram que o offloading para MEC economiza energia e reduz o tempo de processamento de reconhecimento facial. No entanto, a pesquisa se limita a ambientes de teste 4G, restringindo a exploração do verdadeiro potencial do processamento MEC de baixa latência em ambientes 5G.
The proposal presented by \cite{UAV} investigates the potential of Unmanned Aerial Vehicles (UAVs) equipped with IoT devices for facial recognition surveillance at high altitudes. The study demonstrates the viability of offloading video data processing tasks to mobile edge computing (MEC) servers, reducing energy consumption and processing time on board UAVs. The work presents a prototype for facial recognition using the OpenCV Local Binary Pattern Histogram (LBPH) algorithm in a test environment. The results demonstrate that offloading to MEC saves energy and reduces facial recognition processing time. However, the research is limited to 4G test environments, restricting the exploration of the true potential of low-latency MEC processing in 5G environments.

The work \cite{mar_edge} presents an  exploration of MEC as a solution to mitigate the processing delay and energy consumption inherent in mobile augmented reality applications. The authors propose the integration of an edge layer between the user and cloud layers. This design aims to enhance the performance of mobile AR by reducing latency and improving energy efficiency. This study contributes to the future of mobile AR by demonstrating the potential of MEC to enhance the quality of experience (QoE) for AR consumers. The paper uses simulations to evaluate the performance of the proposed hierarchical computation architecture and the results demonstrate that the MEC-based AR framework significantly reduces both energy usage and latency when compared to existing baseline methods, showcasing the effectiveness of the proposed solution for improving mobile AR applications.

Based on the state-of-the-art presented, no articles in the current literature were found to consider 5G, computer vision, and MEC/Cloud integrated in a testbed. In addition, our proposal benefits from a high performance 5G radio, while reducing the overall costs of the deployment using open source solutions for both MEC and the 5G Core, and also the feasibility of integrating a proprietary component with open-source ones in a single end-to-end infrastructure. Therefore, the proposed approach presented in the last row of Table \ref{tab:rel_work} utilizes the MEC and Cloud architecture at the processing layer, employs a computer vision applications through a real 5G testbed.
